EMPOT: partial alignment of density maps and rigid body fitting using unbalanced Gromov-Wasserstein divergence

Aligning EM density maps and fitting atomic models are essential steps in single particle cryogenic electron microscopy (cryo-EM), with recent methods leveraging various algorithms and machine learning tools. As aligning maps remains challenging in the presence of a map that only partially fits the other (e.g. one subunit), we here propose a new procedure, EMPOT (EM Partial alignment with Optimal Transport), for partial alignment of 3D maps. EMPOT first finds a coupling between 3D point-cloud representations, which is associated with their so-called unbalanced Gromov Wasserstein divergence, and second, uses this coupling to find an optimal rigid body transformation. Upon running and benchmarking our method with experimental maps and structures, we show that EMPOT outperforms standard methods for aligning subunits of a protein complex and fitting atomic models to a density map, suggesting potential applications of Partial Optimal Transport for improving Cryo-EM pipelines.

==> macros.tex <==
% \addtolength{\oddsidemargin}{-0.5in}
% \setlength{\evensidemargin}{0in} \setlength{\textwidth}{6.50in}
% \setlength{\textheight}{9.00in } \setlength{\topmargin}{0in}
% \setlength{\headheight}{0in} \setlength{\headsep}{0in}
% % \setlength{\parskip}{\medskipamount}
% \addtolength{\baselineskip}{.5\baselineskip}
%\newtheorem{assumption}{Assumption}
%\newtheorem{proposition}{Proposition}
%\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
%\newtheorem{remark}{Remark}
%\newtheorem{conclusion}{Conclusion}
\newtheorem{acknowledgements}{Acknowledgements}
%\newtheorem{corollary}{Corollary}
\newcommand{\Proof}{\underline{\bf Proof:}}
\newcommand{\Endproof}{~$\Box$~}
%\newcommand{\Remark}{\underline{\bf Remark:~~}}
%\renewcommand{\baselinestretch}{1}
%%%%%%%% the following was suggested by Boaz I hope it works
%\renewcommand{\theequation}{\arabic{section}.\arabic{subsection}...\arabic{equation}}
%\newcommand{\Section}{\setcounter{equation}{0} \section}
\newcommand{\mb}[1]{ \mbox{\boldmath$#1$} }
\newcommand{\ds}{\displaystyle}
% \newcommand{\beq}{\begin{eqnarray}}
% \newcommand{\eeq}{\end{eqnarray}}
% \newcommand{\beqq}{\begin{eqnarray*}}
% \newcommand{\eeqq}{\end{eqnarray*}}
\newcommand{\p}{\partial}
\newcommand{\g}{\gamma}
\newcommand{\eps}{\varepsilon}
\newcommand{\x}{\mbox{\boldmath$x$}}
\newcommand{\n}{\mbox{\boldmath$n$}}
\newcommand{\J}{\mbox{\boldmath$J$}}

%\newcommand{\v}{\mbox{\boldmath$v$}}
\newcommand{\y}{\mbox{\boldmath$y$}}
\newcommand{\z}{\mbox{\boldmath$z$}}

\def\bbP{\mathbb{P}}

\font\bb=msbm10 at 12pt
\font\bbb=msbm10 at 18pt
\def\rR{\hbox{\bb R}}
\def\rN{\hbox{\bb N}}
\def\rQ{\hbox{\bb Q}}
\def\rZ{\hbox{\bb Z}}

\def\frefm#1{{Figure~\ref{#1}}}

\def\fref#1{{Figure~\ref{#1}}}
\def\tref#1{{Table~\ref{#1}}}

\def\edfref#1{\textbf{Extended Data Fig.~\ref{#1}}}
\def\edtref#1{\textbf{Extended Data Table~\ref{#1}}}

\newcommand{\suppfref}[1]{{Figure~\ref{#1}}}
\newcommand{\supptref}[1]{{Table~\ref{#1}}}

\newcommand{\sref}[1]{Section~\ref{#1}}

\def\fixme#1#2{\textbf{[FIXME ({#1}): #2]}}
\def\comment#1#2{\textbf{[COMMENT ({#1}): #2]}}

\newcommand{\beginExtendedData}{%
       \setcounter{section}{0}
       \renewcommand{\thesection}{S\arabic{section}}%
        \setcounter{table}{0}
        \renewcommand{\tablename}{{\bf Extended Data Table}}  
        \renewcommand{\thetable}{{\bf \arabic{table}}}%
        \setcounter{figure}{0}
        \renewcommand{\figurename}{{\bf Extended Data Figure}}    
        \renewcommand{\thefigure}{{\bf \arabic{figure}}}%
     }

\newcommand{\beginSupplement}{%
       \setcounter{section}{0}
       \renewcommand{\thesection}{S\arabic{section}}%
        \setcounter{table}{0}
        \renewcommand{\tablename}{{Table}}  
        \renewcommand{\thetable}{{S\arabic{table}}}%
        \setcounter{figure}{0}
        \renewcommand{\figurename}{{Figure}}    
        \renewcommand{\thefigure}{{S\arabic{figure}}}%
     }     

\renewcommand{\figurename}{\textbf{{Figure}}}        
\def\correction{\rho}
\def\profile{p^\text{exp}}

%\newfloat{Figure 1 supplement}{htbp}{}\floatname{Figure 1 supplement}{Figure~1--Figure Supplement}
%\newcommand{\suppfrefone}[1]{{Figure~1--Figure Supplement~\ref{#1}}}
%
%\newfloat{Figure 2 supplement}{htbp}{}\floatname{Figure 2 supplement}{Figure~2--Figure Supplement}
%\newcommand{\suppfreftwo}[1]{{Figure~2--Figure Supplement~\ref{#1}}}
%
%\newfloat{Figure 3 supplement}{htbp}{}\floatname{Figure 3 supplement}{Figure~3--Figure Supplement}
%\newcommand{\suppfrefthree}[1]{{Figure~3--Figure Supplement~\ref{#1}}}
%
%\newfloat{Figure 4 supplement}{htbp}{}\floatname{Figure 4 supplement}{Figure~4--Figure Supplement}
%\newcommand{\suppfreffour}[1]{{Figure~4--Figure Supplement~\ref{#1}}}
%
%\newfloat{Figure 6 supplement}{htbp}{}\floatname{Figure 6 supplement}{Figure~6--Figure Supplement}
%\newcommand{\suppfrefsix}[1]{{Figure~6--Figure Supplement~\ref{#1}}}
%
%\newfloat{Figure 7 supplement}{htbp}{}\floatname{Figure 7 supplement}{Figure~7--Figure Supplement}
%\newcommand{\suppfrefseven}[1]{{Figure~7--Figure Supplement~\ref{#1}}}


